Reconfiguring Participatory Design to Resist AI Realism

The growing trend of artificial intelligence (AI) as a solution to social and technical problems reinforces AI Realism -- the belief that AI is an inevitable and natural order. In response, this paper argues that participatory design (PD), with its focus on democratic values and processes, can play a role in questioning and resisting AI Realism. I examine three concerning aspects of AI Realism: the facade of democratization that lacks true empowerment, demands for human adaptability in contrast to AI systems' inflexibility, and the obfuscation of essential human labor enabling the AI system. I propose resisting AI Realism by reconfiguring PD to continue engaging with value-centered visions, increasing its exploration of non-AI alternatives, and making the essential human labor underpinning AI systems visible. I position PD as a means to generate friction against AI Realism and open space for alternative futures centered on human needs and values.

==> Paper_Content/4_findings.tex <==
\section{Findings}

We argue for these with two beliefs.
First, AI systems have to align with human values that we collectively negotiate and arrive at through attachments to matters of concern \cite{le2011publics}.
Tensions are bound to arise between AI systems (which include developers and participatory AI practitioners) and the public it purports to support. 
PD has a role to play by ensuring that the public has power and agency to ensure that their values and interests are prioritized. 
Second, AI is not a single unit, it is ecological. It does not occur in isolation. Each AI system taps into and brings with it a myriad of standards, processes, and values, each of which in turn influences our actions and values. 
But despite these infrastructural processes required, AI Realism relies on presenting just the output (e.g., personalization, efficiency, or transparency) while obfuscating the process. 
I believe that this is another place for PD to play a role, by engaging the public with the process, of the 
This complicates the picture of envisioning future possibilities for it necessitates critically seeing the possible long-term impact and broader vision pushed through the AI systems. 
At the same time, 



% revealing the hegemony of forces influencing the setting, reconfiguring aspects of what has been excluded and seeking to include it, and articulating a collective that challenges or provides alternatives to dominant practices 

\subsection{Broadening and Deepening Participation}

In many Participatory AI efforts, participation focuses on inclusion for design input rather than a critical mechanism to support people in setting an agenda. 
The effect of this is that those efforts presuppose AI as a given; the participation is constrained to small-scale inputs on improving the development and deployment of AI \cite{delgado2023participatory}. 
From this perspective, participatory AI is deployed as a mechanism to co-opt human labor toward acquiescence. 
Even in exception cases where the community's voice in deciding whether to use AI is raised (e.g., \cite{ismailkumar, }), constraints such as limited time and resources leave open questions of \emph{how} it can be done. 
Indeed, the opacity and rapid evolution of AI systems raise questions on what even constitutes meaningful participation. 

\citet{bratteteig2018does}, discussing if AI makes PD obsolete, build upon Schön's see-move-see processes \cite{schon1983reflective} to argue for participation in envisioning ideas with knowledge of what AI can and cannot do, concretizing design idea(s) by engaging with values and visions for design, and finally evaluating the impact of the decision. 
While they are valuable steps, these need to be more political. 
Knowing the capabilities, which is a motivation for explainable AI, does not challenge the techno-deterministic stance that it promotes; it still positions our attention to technical solutions rather than engaging in institutional or social possibilities. 
Similarly, engaging with values and visions with participants has the risk of getting consensus on building systems which in reality may necessitate surveillance and other large-scale data collection mechanisms that they were not aware of. 
Seeing how the sausage is made has to be added to the process of participation. 
Further, evaluating the impact of AI systems especially in the design phase is challenging, with effects hidden until development and, often, seen after long-time deployment \cite{bratteteig2016participatory}. 

``Participation becomes a matter of concern, to be assembled and designed, case by case, where the criteria for participation are not transcendent, but carefully developed and explicated in each project'' \cite[pp. 255]{andersen2015participation}, arguing for the construction and reconstruction of participation as a public affair. We concur. 
For PD in the era of AI Realism, the criteria for participation should emphasize enabling agentic decision-making among all stakeholders affected or influencing AI systems and including an agenda of exploring possibilities \emph{without} AI.  
As PD practitioners, we have a responsibility  \cite{bratteteig2012disentangling}.
To this end, in participatory AI engagements, we need to focus on empowering broader stakeholders in the decision-making process where they have the agency to (1) generate friction to ask whether AI is even needed by placing AI solutions against other technical and social alternatives, (2) surface (mis)alignments between the values espoused and the values demanded in realizing the AI solution(s), and (3) delineate boundaries for AI approach and devising mechanisms to enforce the boundaries in the long run. 
% As actors who initiate the PD engagement, building these into our approach is our responsibility \cite{bratteteig2012disentangling}. 

% Shouldn't I be talking about community governance and commoning?


\subsection{Questioning Personalization: Reevaluating Mutual Learning}
% Human malleability and machine intransingence

Personalization is one of the most visible aspects of the use of AI among the masses, with product and content recommendations, advertisement placements, and email generation being commonplace.
In fact, personalization through AI has been pushed to such an extent that a 2021 McKinsey and Company report states, ``Consumers don’t just want personalization, they demand it.'' \cite{mckinseyHyperPersonalization}. 
Particularly to support personalization, AI systems are constantly collecting data leading to a situation where they are being trained when they are being used \cite{bratteteig2018does}.
This training-in-use paradigm obfuscates the AI system's processes and impact, surfacing tensions with PD's value in mutual learning.

% There are two major problems we see: (1) users tend to adapt -- human malleability and (2) machines tend to solidify their perspective about us, leaving little room for us to change. 
% Mutual learning presupposes a process of negotiating and arriving at values that align between the stakeholders. 
I see the tension emerging in two directions.  
First, personalization in AI systems demands human malleability.
This is not a new phenomenon: people accommodate technology by changing their behavior and practices around the technology \cite{}.
But with AI, the accommodation demanded involves both in using the AI and, since AI is trained in use, in training the AI where human flexibility further reifies its assumptions, leaving little room for alternatives.
\citet{gyldenkaerne2020pd}, for example, in studying AI use in electronic health records in Denmark, highlight how an AI system imposed a new process of data collection even though the clinician's existing processes were sufficient for their purposes. It not only changed the way clinicians recorded patient data but since it was rife with ambiguity, made additional demands on the clinicians to attend to the data processes. 
%Second, AI systems enforce a perspective about us and the world, leaving little room for us to change it. 
%In the case of the clinicians, despite the mismatch in their practices and the new AI-based processes, they did not have a room for recourse; they had to devise additional workarounds \cite{gyldenkaerne2020pd}.
Moreover, the clinicians did not have room for recourse; they had to devise additional workarounds \cite{gyldenkaerne2020pd}.
In many respects, it is a classic challenge that PD has grappled with -- ensuring that users gain control over the tools and their environment \cite{bratteteig2016participatory}.


Second, personalization erodes opportunities for finding common ground, raising challenges for surfacing shared experiences and engaging in collective action.
%How do we learn from each other's experiences when each of us is experiencing differences because of personalization?
We are forced to work on pushing back on the limitations and impositions of our own spaces rather than drawing commonalities among a larger mass to push against the system.
This echoes the Marxist notion of ideology---that AI systems are \emph{the} thing---and acquiescing the alienation that it brings.  
A significant exercise of abstraction is necessary to arrive at shared experiences and enable mutual learning; these skills are not easily accessible to all.
For PD, which relies on forming publics---of people forming attachments to shared matters of concern---this is a new challenge, and one that I believe PD ought to undertake.  

Given the power differences between those who own the AI system and those who are affected by it, a way forward for PD would be to take an agonistic stance and support the creation of counter-structures and alternatives. 
The alternatives ought to involve non-AI systems for any AI system, even if it is critical of the existing system, enforces the belief that AI is the natural order. 
The alternative non-AI design may not necessarily lead to the refusal of AI but it affords two critical aspects. First, it allows us to critically reflect and distill aspects of the users' needs and the situation that truly requires AI solutions. 
Second, in thinking about a non-AI alternative, we create space to reflect on the human labor that is assumed and becomes necessary for the AI to function.




\subsection{Questioning Efficiency: Envisioning Alternative Future Possibilities}
% Human labor behind the work 

Despite the allure of magical-seeming machine intelligence, the reality in AI systems is that the critical infrastructure underlying it all---collecting, cleaning, and labeling data---relies on human labor. 
The labor is typically sourced out to the Global South where worker conditions and compensations are, at best, questionable (e.g., \cite{wang2022whose, williams2022exploited}).
The indispensable human labor is obfuscated behind claims of technological progress of AI.
Ironically, the very same AI that has relied on the labor of the many is used to justify promoting efficiency by laying off employees elsewhere \cite{thorbecke2024tech}.
%A prominent example of this is the recent Duolingo layoff where the workers at most precarious positions were laid off citing AI-enabled efficiency\footnote{\url{https://www.washingtonpost.com/technology/2024/01/10/duolingo-ai-layoffs/}}.

There are two facets to the problem.
First, the promotion of AI's efficient capabilities hides the large human labor that has been put into place to realize it. 
Those who use and are affected by AI are placed at a distance from those who build the infrastructure for that AI, enabling very little space for collective action and solidarity.  
Second, ``efficiency'' is presented as the only metric that should guide our endeavors. 
It leaves no room to explore alternative visions that we could collectively design \cite{huybrechts2020visions}. 


PD can play a role in attending to these issues.
A way forward is for PD to support collective action, particularly by bringing together the precarious workers early in the AI development pipeline and the higher-paid, slightly-empowered workers---as the recent layoffs suggest no worker is truly in control---in solidarity \cite{williams2022exploited}.
Design, here, invokes configuring the social processes towards change rather than a technological reconfiguration.
Second, PD methods can be structured to surface the hidden labor behind the AI systems as well as the malleability demanded of the AI users. 
Latour, using a door as an exemplary technology, expounds on the value of ``delegation'', i.e., the work the technology does that humans no longer have to do \cite{johnson1988mixing}. 
I contend that for ecological technology like AI, PD methods have to engage with ``delegation inversion'', the additional work and sacrifice humans have to make for the technology to function. 



%It is akin to Star's strategy of studying an infrastructure by studying the hidden labor enabling and maintaining it. 




% Make the labor behind the infrastructure that is being used to construct AI solutions visible so that there is friction in considering whether it is truly necessary.


% Our approach seeks to deal with the micro-relations and interactions at an individual and organizational level, designing a vision \cite{huy2020visions} to bring change on the big issue (i.e., of the politics in the organization) but by paying attention to the individual relations and interactions. 

% ``Our hypothesis is that designing ‘visions’ can turn the tension between addressing the focus on the big issues and the close attention to the particularity of relations into a dynamic dialogue that can repoliticise design.'' \cite{huybrechts2020visions}
% ``when visions on the big issues are kept in the picture in this relational work, politics is back to the centre stage'' 

% Why do the configurations matter -- the situated nature of design and its challenges in dealing with large scale politics. The politicization we see builds on Swyngedouw's notion of  ``articulation of divergent, conflicting, and alternative trajectories of future […] possibilities and assemblages'' \cite{swyngedouw2007post}. Building on post-colonial computing \cite{irani2010post}, the politics of design requires attention to the work revolving around engagement (e.g., who is participating and how), articulation (e.g., what conditions lead to our identification of assets), and translation (e.g., how are the assets and the broader context informing design decisions).










% Enderud (1981) look at conflicts and how different ways of structuring and controlling help avoid addressing these conflicts. The mechanisms they identified are: agenda control (what is discussed and who decides the themes), participants (who are invited in), scope (which solutions are possible – and hence, which problems are defined and seen as relevant and therefore addressed), and resources (available time and people). 




%     There is a lack of clarity and consensus on what meaningful participation entails, as well as standards for assessing participatory mechanisms (Birhane et al., 2022).
%     Participatory efforts often confront tensions between aspirations for stakeholder empowerment and practical constraints like limited resources, timelines, and incentives (Delgado et al., 2023).
%     Without careful design, participatory initiatives risk being extractive, tokenistic, or washing over true power imbalances (Birhane et al., 2022; Bødker & Kyng, 2018).
%     The opacity and continual evolution of AI systems pose challenges for meaningful human participation, interpretation, and oversight (Birhane et al., 2022; Bødker & Verne, 2018).
%     Scaling participation to the spatial and temporal dimensions of big data and AI systems remains an open challenge (Birhane et al., 2022; Delgado et al., 2023).


% While Bødker, Ehn, Kyng et al. (1987) emphasized alternative technological futures through methods like mockups and roleplaying, their later assessment concedes that workers gained little actual control or ownership from these visions. This prompts questions on participatory AI - what constitutes meaningful control or ownership for stakeholders over opaque, continually evolving algorithmic systems? Are current approaches genuinely empowering?

% Bratteteig & Wagner (2016) argue that most participatory decision-making involves narrow choices within predefined constraints by experts. This risks pseudo-participation that extracts input while blocking deeper challenges to agendas and power structures. Similar risks persist in participatory AI. How can participatory mechanisms move from merely consulting on interfaces to shaping fundamental system purpose and value functions? Can participation transform the politics shaping what gets automated?


% Deliberating with AI: Improving Decision-Making for the Future through Participatory AI Design and Stakeholder Deliberation by Zhang et al. (CHI 2023)


%     Lack of accountability and oversight in AI-enabled surveillance

% Case: Predictive policing systems that leverage machine learning to forecast crime hotspots are being deployed in cities like Chicago with little governance or independent auditing (Birhane et al., 2022). These opaque systems risk perpetuating systemic biases against marginalized groups and violate civil liberties through unrestrained surveillance.

% Connection: This shows the push towards AI-enabled surveillance without accountability mechanisms or concern for potential misuse. There is a lack of public oversight over these predictive systems that deeply impact people's lives.

% Participatory Possibility: Impacted communities could be engaged through participatory design workshops to shape auditing practices for AI predictive policing models. This could give citizens voice in determining metrics and processes for evaluating systems.

%     Socially shaped algorithms demanding human adaptability

% Case: YouTube's algorithmic recommendation models pressure content creators to produce videos tailored towards maximizing watch time and platform incentives, rather than creative goals (Delgado et al., 2023). This obscures that YouTube's algorithms embody particular design choices and incentives.

% Connection: In this case, human behavior and creativity is constrained by algorithms optimized for platform objectives. It presents a refusal to shape algorithms to creative needs.

% Participatory Possibility: YouTubers and viewers could participate in deliberative workshops to determine value metrics and objectives for YouTube's recommendation algorithms beyond simply maximizing engagement.

%     Invisibilized human labor subsidizing promises of AI efficiency

% Case: Large language models like GPT-3 were enabled by vast datasets of text labeled through exploitative crowd work. But narratives on AI progress focus on computational power rather than this hidden labor (Birhane et al., 2022).

% Connection: This exemplifies the indispensable human work that is invisibilized behind claims of autonomous technical achievement in AI. Crowd workers' contributions are unrecognized and uncompensated.

% Participatory Possibility: Data labeling and enrichment could become recognized as valued work through worker-centered participatory design of ethical crowdsourcing platforms. This would focus on the interests of crowd workers themselves in system design.

%     Lack of meaningful participation in algorithmic governance

% Case: Facebook content moderators have little power in platform governance or recourse against mental health consequences from moderation work, despite their crucial role (Delgado et al., 2023).

% Connection: Content moderators exemplify how workers subsidizing AI systems can be excluded from platform decision-making and given no voice in governance.

% Participatory Possibility: Participatory mechanisms could involve content moderators along with impacted user groups in oversight boards that govern aspects of platforms like content policies and appeals processes. This would give moderators agency in platform governance.


==> Paper_Content/question_list.tex <==
How can participatory mechanisms move from merely consulting on interfaces to shaping fundamental system purpose and value functions? Can participation transform the politics shaping what gets automated?
